SLIM: Explicit Slot-Intent Mapping with BERT for Joint Multi-Intent Detection and Slot Filling

Utterance-level intent detection and token-level slot filling are two key tasks for natural language understanding (NLU) in task-oriented systems. Most existing approaches assume that only a single intent exists in an utterance. However, there are often multiple intents within an utterance in real-life scenarios. In this paper, we propose a multi-intent NLU framework, called SLIM, to jointly learn multi-intent detection and slot filling based on BERT. To fully exploit the existing annotation data and capture the interactions between slots and intents, SLIM introduces an explicit slot-intent classifier to learn the many-to-one mapping between slots and intents. Empirical results on three public multi-intent datasets demonstrate (1) the superior performance of SLIM compared to the current state-of-the-art for NLU with multiple intents and (2) the benefits obtained from the slot-intent classifier.

==> text/2-related.tex <==
\section{Related Work}
%%% related work需要好好大改 先对两个task传统方法进行简单总结，再对近期效果比较好的和相关的方法进行相对多一点点的review，再对joint方法说一下。后两者，试着说下之前方法有什么不足之处，尽量过渡和我们的connect一下。
\FY{Related work could be removed?} \MF{Definitely not, this is quite important.}
Intent detection and slot filling are two major task for spoken language understand in task-oriented dialog system.
For intent detection, SVM \citep{haffner2003optimizing}, CNN \citep{DBLP:conf/emnlp/Kim14}, LSTM \citep{ravuri2015recurrent}, and multiple variants \MF{detail the variants} \citep{DBLP:conf/interspeech/ZhaoW16, DBLP:conf/naacl/YangYDHSH16} are proposed.

Methods such as Markov sequential models \citep{DBLP:journals/coling/BergerPP96}, CRF \cite{DBLP:conf/icml/LaffertyMP01}, CNN \citep{DBLP:conf/interspeech/Vu16}, and LSTM \citep{DBLP:conf/slt/YaoPZYZS14} are put forward to address the slot filling problem.

Jointly modeling of two tasks \cite{DBLP:conf/interspeech/LiuL16, DBLP:conf/naacl/GooGHHCHC18, DBLP:conf/emnlp/LiuMZZCX19} demonstrates an intuitive and popular direction in research since it captures the internal semantic dependency. Due to the scarcity of useful SLU datasets,  \citet{DBLP:journals/corr/JointBert} first utilizes the large-scale pretrained language model, BERT \citep{DBLP:conf/naacl/DevlinCLT19}, to improve the model's generalization capability.

Above methods simplify and treat the intent detection as a single-label problem. \citet{DBLP:conf/asru/XuS13, DBLP:journals/mta/KimRL17} extend the formulation to a multi-label classification problem. \citet{DBLP:conf/naacl/GangadharaiahN19} further incorporates the joint modeling which learns a multi-intent classifier and slot filling model simultaneously and evaluates the model on an internal dataset. \citet{DBLP:conf/emnlp/QinXCL20} exploits more fine-grained intent information and also publishes two artificial multi-intent SLU datasets constructed by combining utterances from traditional single-intent datasets. 

